Quantitative Games on Probabilistic Timed Automata

Two-player zero-sum games are a well-established model for synthesising controllers that optimise some performance criterion. In such games one player represents the controller, while the other describes the (adversarial) environment, and controller synthesis corresponds to computing the optimal strategies of the controller for a given criterion. Asarin and Maler initiated the study of quantitative games on (non-probabilistic) timed automata by synthesising controllers which optimise the time to reach a final state. The correctness and termination of their approach was dependent on exploiting the properties of a special class of functions, called simple functions, that can be finitely represented. In this paper we consider quantitative games over probabilistic timed automata. Since the concept of simple functions is not sufficient to solve games in this setting, we generalise simple functions to so-called quasi-simple functions. Then, using this class of functions, we demonstrate that the problem of solving games with either expected reachability-time or expected discounted-time criteria on probabilistic timed automata are in NEXPTIME $\cap$ co-NEXPTIME.

==> mdp.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\section{Stochastic Games}
\label{Sec:stochastic-games}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{definition}
  A \emph{Markov decision process} is a tuple  $\mdp = (S, A, p, \pi)$
  where: 
  \begin{itemize}
  \item
    $S$ is the set of \emph{states}; 
  \item
    $A$ is the set of \emph{actions};
  \item
    $p : S \times A \to \DIST(S)$ is a partial function called the
    \emph{probabilistic transition function};
  \item
    $\pi: S {\times} A \to \Rplus$ is a bounded and measurable
    \emph{price function} assigning positive real-values to
    state-action pairs. 
  \end{itemize}
\end{definition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\Ashu{Say that in general one can consider nonpositive values as well}

We write $A(s)$ for the set of actions available at $s$, i.e., the
set of actions $a$ for which $p(s, a)$ is defined. 
For technical convenience we assume that $A(s)$ is nonempty for all 
$s \in S$.
We say $\mdp$ is finite, if the sets $S$ and $A$ are finite. 

The \emph{arena} for a \emph{stochastic game} is a triplet $\Mm = 
(\mdp, S_\mMIN, S_\mMAX)$, where $\mdp = (S, A, p, \pi)$ is an MDP and
$(S_\mMIN, S_\mMAX)$ is a partition of $S$.
Intuitively $S_\mMIN$ is the set of states controlled by player Min,
and $S_\mMAX$ is the set of states controlled by player Max.
In a stochastic game on $\Mm$ players Min and Max
move a token along the states of the MDP in the following manner. 
If the current state is $s$, then the
player controlling the state chooses an action $a \in A(s)$ after
which a probabilistic transition is made according to the distribution
$p(s,a)$, i.e., state $s' \in S$ is reached with probability  
$p(s'|s, a) \rmdef p(s, a)(s')$.
In the next turn the player controlling the state $s'$ chooses an
action in $A(s')$ and a probabilistic transition is made accordingly. 
We say that $(s, a, s')$ is a transition in $\Mm$ if 
$p(s' | s, a) {>} 0$ and a \emph{play} of $\Mm$ is a sequence  
$\seq{s_0, a_1, s_1, \ldots} \in S {\times} (A {\times} S)^*$
such that $(s_i, a_{i+1}, s_{i+1})$ is a transition for all 
$i {\geq} 0$. 
We write $\RUNS^\Mm$ ($\FRUNS^\Mm$) for the sets of infinite (finite) 
plays and $\RUNS^\Mm(s)$ ($\FRUNS^\Mm(s)$) for the
sets of infinite (finite) plays starting from state~$s$. 
For a finite play $r {=} \seq{s_0, a_1, \ldots, s_n}$ we write
$\LAST(r) {=} s_n$ for the last state of the play. 
Furthermore, let $X_i$ and $Y_i$ denote the random variables
corresponding to $i^{\text{th}}$ state and action of a run. 

A \emph{strategy} of player Min in $\Mm$ is a partial function 
$\mu: \FRUNS^\Mm \to \DIST(A)$ such that for a finite play $r \in
\FRUNS^\Mm$ the function $\mu(r)$ is defined if $\LAST(r) \in S_\mMIN$
and it is such $\supp(\mu(r)) \subseteq A(\LAST(r))$. 
Similarly a strategy of player Max is defined.
We write $\Sigma^\Mm_\mMIN$ and $\Sigma^\Mm_\mMAX$ for the set of
strategies of player Min and player Max, respectively.
Let $\RUNS^\Mm(s, \mu, \chi)$ denote the subset of $\RUNS^\Mm(s)$
which correspond to the set of runs starting from $s \in S$ where
Min and Max play according to strategies $\mu$ and $\chi$,
respectively. 

We say that a strategy $\sigma$ is \emph{pure} if $\sigma(r)$ is a 
point distribution for all  $r \in \FRUNS^\Mm$.
We say that a strategy $\sigma$ is \emph{stationary} if $\LAST(r) {=}
\LAST(r')$ implies $\sigma(r) {=} \sigma(r')$ for all 
$r, r' \in \FRUNS^\Mm$. 
A strategy $\sigma$ is \emph{positional} if it is both pure and
stationary. 
To analyse the behaviour of a stochastic game on $\Mm$ under a
strategy pair $\mu \in \Sigma^\Mm_\mMIN$ and $\chi \in
\Sigma^\Mm_\mMAX$, for each state $s$ of $\Mm$, we define a
probability space 
$(\RUNS^\Mm(s, \mu, \chi), \mathcal{F}_{\RUNS^\Mm(s, \mu,
  \chi)},\PROB^{(\mu, \chi)}_s)$ over the set of infinite runs under
strategies $\mu$ and $\chi$ with $s$ as the initial state. 
For details on this construction see, for example, \cite{Put94}. 
Given a \emph{real-valued random variable} over the set of infinite
runs $f : \RUNS^\Mm \to \Real$, using standard techniques from
probability theory, we can define the expectation  of this variable
$\eE^{(\mu, \chi)}_s\set{f}$ with respect to strategy pair $(\mu,
\chi)$ when starting in $s$.  
%For an infinite run $r = \seq{s_0, (t_1, a_1), s_1, \ldots}$ we define
%$\STOP(r) = \inf \set{i \::\: s_i \in F}$. 
%In this paper we work with the following assumptions
%\begin{remark}
%  For every run $r \in \RUNS$ we assume that $\STOP(r) < \infty$. 
%\end{remark}

\subsubsection{Performance objectives.}
For a stochastic game on $\Mm=(\mdp, S_\mMIN, S_\mMAX)$, under
any strategy pair $(\mu, \chi)$ and starting from any state $s$, there
is a sequence of random prices $\{ \pi(X_{i-1},Y_i) \}_{i \geq 1}$.
Depending on the stochastic game under study there are a number of
different performance objectives that can be studied. 
Below are the objectives most often used.
\begin{enumerate}
\item
  \emph{Expected Reachability Price} (with \emph{target set} $F$):
  \[
  \EREACHPRICE_{\Mm}(F)(s, \mu, \chi) \rmdef
  \eE^{(\mu, \chi)}_s
  \left\{\mbox{$\sum_{i=1}^{\min \set{i \, | \, X_i \in F}}$} 
    \pi(X_{i-1}, Y_{i}) \right\}.
  \]
\item
  \emph{Expected Discounted Price} (with \emph{discount factor}
  $\lambda \in (0, 1)$): 
  \[
  \EDISCTPRICE_{\Mm}(\lambda)(s, \mu, \chi) \rmdef
  \eE^{(\mu, \chi)}_s \left\{
    (1{-}\lambda) \mbox{$\sum_{i=1}^\infty$} 
    \lambda^{i-1} \pi(X_{i-1}, Y_i) \right\} \, .
  \]
\item
  \emph{Expected Average Price:}
  \[
  \EAVERAGEPRICE_{\Mm}(s, \mu, \chi) 
  \rmdef \limsup_{n \to \infty} 
  \frac{1}{n} \eE^{(\mu, \chi)}_s 
  \left\{ \mbox{$\sum_{i=1}^{n}$} \pi(X_{i-1}, Y_i) \right\}.
\] 
\end{enumerate}

For an objective $\EPRICE_\Mm$ and state $s$ we define its lower value
$\LEPRICE(s)$ and upper value $\UEPRICE(s)$ as follows:
\begin{eqnarray*}
  \LEPRICE(s) & = & \sup_{\chi \in \Sigma_\mMAX} \inf_{\mu \in
    \Sigma_\mMIN} \EPRICE_\Mm(s, \mu, \chi), ~\text{ and
  } \\
  \UEPRICE(s) & = & \inf_{\mu \in \Sigma_\mMIN} \sup_{\chi \in
    \Sigma_\mMAX} \EPRICE_\Mm(s, \mu, \chi). 
\end{eqnarray*}
It is easy to verify that for any performance objective  for all $s
\in S$ we have that
$\LEPRICE(s) \leq \UEPRICE(s)$.  
We say that game is determined if $\LEPRICE(s) = \UEPRICE(s)$ for all
$s \in S$. 
In this case we also say that the value of the game exists and denote
it by $\EPRICE(s) = \LEPRICE(s) = \UEPRICE(s)$ for all $s \in S$.

For strategies $\mu \in \Sigma^\Mm_\mMIN$ and $\chi \in
\Sigma^\Mm_\mMAX$, we define 
\begin{eqnarray*}
\EPRICE^\mu(s) &=& \sup_{\chi \in \Sigma^\Mm_\mMIN} 
\EPRICE_\Mm(s, \mu, \chi), \text{ and } \\
\EPRICE_\chi(s) &=& \inf_{\mu \in \Sigma^\Mm_\mMIN} 
\EPRICE(s, \mu, \chi).
\end{eqnarray*}
For an $\varepsilon > 0$, we say that a strategy 
$\mu \in \Sigma^\Mm_\mMIN$ or $\chi \in \Sigma^\Mm_\mMAX$ is 
\emph{$\varepsilon$-optimal} if for every $s \in S$, we have
$\EPRICE^\mu(s) \leq \EPRICE(s) + \varepsilon$ or 
$\EPRICE_\chi(s) \geq \EPRICE(s) - \varepsilon$, respectively. 
Note that if a stochastic game is determined then for every
$\varepsilon > 0$, both players have $\varepsilon$-optimal strategies.

We say that a stochastic game is \emph{positionally determined}
if for every~$s \in S$, we have  
$\EPRICE(s) = \inf_{\mu \in \Pi^\Mm_\mMIN} \sup_{\chi \in
  \Sigma^\Mm_\mMAX} \EPRICE_\Mm(s, \mu, \chi)$
and 
$\EPRICE(s) = \sup_{\chi \in \Pi^\Mm_\mMAX} \inf_{\mu \in
  \Sigma^\Mm_\mMIN}  \EPRICE_\Mm(s, \mu, \chi)$.
Note that if a stochastic game is positionally determined
then for every $\varepsilon > 0$, both players have \emph{positional} 
$\varepsilon$-optimal strategies. 

\Ashu{Check if we call runs plays everywhere.}

For technical convenience we make the follows assumptions for
reachability objectives \cite{dA99}. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assum}
  \label{assum:absorbing}
  If $s \in F$, then $s$ is 
  \emph{absorbing}
  and \emph{cost free}, i.e. $p(s|s,a) {=} 1$ and $\pi(s, a) {=} 0$ for
  all $a \in A(s)$. 
\end{assum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{assum}
  \label{assum:proper-strategy}
  For every strategy pair $\mu \in \Sigma^\Mm_\mMIN$, $\chi \in
  \Sigma^\Mm_\mMAX$, and state $s \in S$ we have that 
  $\lim_{i \to \infty} \PROB^{(\mu, \chi)}_s(X_i \in F) = 1$. 
\end{assum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsubsection{Optimality Equations.}
We now review optimality equations for characterising the value in the
games given above.  
\begin{enumerate}
\item (Expected reachability-price game.)
  Let $P : S \to \Real$ and $F \subseteq S$; we write 
  $P \models \ROpt^F(\Mm)$, and we say that $P$ is a solution of
  optimality equations $\ROpt^F(\Mm)$ if, for all $s \in S_\mMIN$, we
  have: 
  \[
  P(s) = 
  \left\{ \begin{array}{cl}
      0 & \mbox{if $s \in F$}\\
      \inf_{a \in A(s)} \left\{ \pi(s,a) + \sum_{s' \in S} p(s'|s, a)
        \cdot P(s') \right\} & \mbox{otherwise}
    \end{array} \right.
  \]
  and for all $s \in S_\mMAX$, we have:
  \[
  P(s) = 
  \left\{ \begin{array}{cl}
      0 & \mbox{if $s \in F$}\\
      \sup_{a \in A(s)} \left\{ \pi(s,a) + \sum_{s' \in S} p(s'|s, a)
        \cdot P(s') \right\} & \mbox{otherwise}
    \end{array} \right.
  \]
\item (Expected discounted-price game.)
  Let $D : S \to \Real$; we write $D \models \DOpt(\Mm)$, and we say
  that $D$ is a solution of optimality equations $\DOpt(\Mm)$ if, for
  all $s \in S_\mMIN$, we have:  
  \[
  D(s) = \inf_{a \in A(s)}
  \left\{ (1{-}\lambda) \cdot \pi(s,a) +  \lambda \cdot 
    \mbox{$\sum_{s' \in S}$} p(s'|s, a) \cdot D(s') \right\}
  \]
  and for all $s \in S_\mMAX$, we have:  
  \[
  D(s) = \sup_{a \in A(s)}
  \left\{ (1{-}\lambda) \cdot \pi(s,a) +  \lambda \cdot 
    \mbox{$\sum_{s' \in S}$} p(s'|s, a) \cdot D(s') \right\}
  \]
  
\item (Expected average-price game.)
  Let $G : S \to \Real$ and $B: S \to \Real$; we write 
  $(G, B) \models \AOpt(\Mm)$, and we say that  
  $(G, B)$ is a solution of optimality equations\footnote{These
    optimality equations are slightly different from Howard's
    optimality equations for expected average price, and correspond
    to Puterman's~\cite{Put94} modified optimality equations.} 
  $\AOpt(\Mm)$, if for all $s \in S_\mMIN$, we have: 
  \begin{eqnarray*}
    G(s) & = & \inf_{a \in A(s)} \left\{ 
      \mbox{$\sum_{s' \in S}$} p(s'|s, a) \cdot G(s') \right\}\\
    B(s) & = & \inf_{a \in A(s)} \left\{ 
      \pi(s,a) - G(s) + 
      \mbox{$\sum_{s' \in S}$}  p(s'|s, a) \cdot B(s') \right\}
  \end{eqnarray*}
  
  and for all $s \in S_\mMAX$, we have: 
  \begin{eqnarray*}
    G(s) & = & \sup_{a \in A(s)} \left\{ 
      \mbox{$\sum_{s' \in S}$} p(s'|s, a) \cdot G(s') \right\}\\
    B(s) & = & \sup_{a \in A(s)} \left\{ 
      \pi(s,a) - G(s) + 
      \mbox{$\sum_{s' \in S}$}  p(s'|s, a) \cdot B(s') \right\}
  \end{eqnarray*}
\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
The proof of the following proposition is routine and for details see,
for example, \cite{DY79}. 
\begin{proposition}
  \label{prop:oe-give-opt-reach}
  Let $\Mm$ be a stochastic game arena.
  \begin{enumerate}\addtolength{\itemsep}{3pt}
  \item
    If $P {\models} \ROpt^F(\Mm)$, then 
    $P(s) {=} \EREACHPRICE_\Mm(F)(s)$ for all $s\in S$. 
  \item 
    If $D {\models} \DOpt(\Mm)$ and $D$ is bounded, then 
    $D(s) {=} \EDISCTPRICE_\Mm(\lambda)(s)$ for all $s\in S$. 
  \item
    If $(G, B) {\models} \AOpt(\Mm)$ and $G, B$ are bounded,
    then $G(s) {=} \EAVERAGEPRICE_\Mm(s)$ for all $s\in S$. 
  \end{enumerate}
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Notice that, for each objective, if, for every state $s \in S$, the
infimum and supremum, as aplicable, is attained in the optimality
equations, then there exists an optimal positional strategy.
An important class of stochastic game arenas with this property are
stochastic games on finite MDPs, which gives us the following
proposition. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proposition}
  % [Existence of a Solution Implies Positionality in Finite MDPs]
  \label{prop:sol-implies-positional}
  For every finite stochastic game arena, the existence of a solution
  of the optimality equations for the expected reachability,
  discounted and average price implies that the corresponding
  stochastic game is positionally determined.
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
For a finite stochasitc game arena $\Mm$ a solution of optimality
equations for expected reachability, discounted, and average
price objectives can be obtained by value iteration or strategy
improvement algorithms \cite{FV97}. 
The termination of the strategy improvement algorithm is guaranteed as
there are finitely many positional strategies in a finite stochastic
game arena. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{proposition}
  \label{prop:existence-of-solution}
  For every finite stochastic game arena, there exist solutions of the
  optimality equations for expected reachability, discounted,
  and average price objectives.  
\end{proposition}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
Proposition~\ref{prop:sol-implies-positional} together with 
Proposition~\ref{prop:existence-of-solution} provide a proof of 
the following well-known result for stochastic games \cite{FV97}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
\begin{theorem}[Positional Determinacy]
  \label{theorem:finite-positional-optimality}
  For a finite stochastic game arena the expected reachability,
  discounted, and average price games are positionally determined. 
\end{theorem}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

\subsection{Expected Reachability-Time Games}

The performance objectives discussed in
Section~\ref{Sec:stochastic-games} give rise to corresponding
stochastic games on probabilistic timed automata.
Since the price of an action in a probabilistic timed automaton is
equal to the time associated with that action, we call the games
corresponding to expected reachability-price, discounted-price, and
average-price objectives as expected reachability-time, expected
discounted-time, and expected avergae-time games, respectively.  
On the other hand, we call the corresponding games on timed automata
as reachability-time games, discounted-time games, and average-time
games. 

Asarin and Maler gave a value iteration algorithm to solve
reachability-time  games for strongly non-Zeno timed automata.
They proposed a special class of functions, called simple functions,
and using the properties of these functions they proved correctness
and termination of their algorithm.
Jurdzi{\'n}ski and Trivedi extended their work by giving a strategy
improvement algorithm to solve reachability-time games on arbitrary
timed automata and also gave the exact complexity of solving these
games.
They proposed an abstraction of timed automata, a weighted graph
called boundary region graph, and showed that if the solution of
optimality equations for reachability-time objective is a regionally
\Ashu{Region is not yet defined!}
simple function (i.e. can be represented as a function from regions to
simple functions), then it gives a solution of optimality equations
for the reachability-time objective on timed automata.

\begin{theorem}[\cite{AM99,JT07}]
  Reachability-time games are positionally determined, and the exact
  complexity of solving reachability-time games in EXPTIME-complete
  for timed automata with two or more clocks. 
\end{theorem}

Simple functions were also shown to be useful in the reduction of
average-time game to solving mean payoff game on the corresponding
boundary region graph. 

\begin{theorem}[\cite{JT08b}]
  Average-time games are determined, and the exact complexity of
  solving average-time games in EXPTIME-complete for timed
  automata with two or more clocks.  
\end{theorem}

However, we are not aware of any result on the decidability of
discounted-time games. 

Recently~\cite{JKNT09} we extended boundary region graph construction
for probabilistic timed automata and using that we showed that
a number of one-player games on probabilistic timed automata can be
reduced to solving similar games on the corresponding boundary region
graph.
In this paper we show that expected reachability-time game and
expected discounted-time game on probabilistic timed automata can be
reduced to solving similar games on the corresponding boundary region
graph. 
The following is the main result of the paper:

\begin{theorem}
  Expected reachability-time games and expected discounted-time games
  are positionally determined, and the complexity of solving
  these games is in NEXPTIME $\cap$ co-NEXPTIME. 
  Moreove, these games are EXPTIME-hard on probabilistic timed
  automata with two or more clocks. 
\end{theorem}

As a side-result we show the following result for discounted-time
games. 

\begin{theorem}
  Discounted-time games are positionally determined, and the
  complexity of solving discounted-time games is EXPTIME-complete on
  timed automata with two or more clocks. 
\end{theorem}

Unfortunately the techniques presented in this paper do not carry
over to solve expected average-time games.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
% If $(\ell, \nu) \in S$ and $c \in C$, then we write $(\ell,\nu)(c)$ for
% $\nu(c)$. \gethin{not sure this is needed any more}
% For a configuration $(\ell, \nu) \in Q$ and $t \in \Rplus$, we
% define $(\ell,\nu) + t$ to be the configuration $(\ell, \nu + t)$.
% and we then write $(\ell,\nu) \xrightharpoonup{}_t (\ell',\nu+t)$.  
% We write $(\ell,\nu) \xrightarrow{}_t (\ell,\nu+t)$ if 
% $(\ell,\nu) \xrightharpoonup{}_t (\ell,\nu+t)$ and 
% for all $t' \in [0, t]$, we have $\nu + t' \sat \inv(\ell)$. 
% 
%\Ashu{Do we really need this assumption?}
%We assume the following---standard and easy to
%syntactically verify---restriction on PTAs which ensures
%\emph{time divergent} behaviour. 
%\begin{assum}
%  We restrict attention to \emph{structurally
%    non-Zeno} probabilistic timed automata~\cite{Tri99,JLS08}. A PTA 
%is structurally non-Zeno if, for any run   
%  $\seq{s_0, (t_1, a_1), \dots, s_n}$, 
%  such that $s_0 {=} (\ell_0, \nu_0)$, $s_n {=} (\ell_n, \nu_n)$ and  
%  $\ell_0 {=} \ell_n$ (i.e., the run forms a cycle in the 
%  finite graph of the locations and transitions of the automaton) we have $\sum_{i=1}^n t_i \geq 1$. 
%\end{assum}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 



    \begin{multline*}
      |F^\oplus_{\alpha,\lambda}(\nu_1) -
      F^\oplus_{\alpha,\lambda}(\nu_2)|\\
      = |b - \nu_1(c) + \lambda \cdot F(\SUCC(\nu_1, \alpha)) 
      - (b - \nu_2(c)) - \lambda \cdot F(\SUCC(\nu_2, \alpha))|\\
      = |(\nu_2(c) - \nu_1(c)) + \lambda \cdot (F(\SUCC(\nu_1, \alpha)) 
      -  F(\SUCC(\nu_2, \alpha)))|\\
      \leq |(\nu_2(c) - \nu_1(c))| (1 + \lambda)\\
      = |\lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha)))|\\
      \leq \lambda \cdot k \cdot \InfNorm{\SUCC(s_1, \alpha) -
        \SUCC(s_2, \alpha)}\\
      = \lambda \cdot k \cdot d
      = \lambda \cdot k \cdot \InfNorm{s_1 - s_2}
    \end{multline*}
    
    If $s_1(c) = s_2(c)$ then $\SUCC(s_1, \alpha) \leq \SUCC(s_2,
    \alpha)$ and moreover $\SUCC(s_2, \alpha) = \SUCC(s_1, \alpha) + d$.
    \begin{multline*}
      |F^\oplus_{\alpha,\lambda}(s_1) -
      F^\oplus_{\alpha,\lambda}(s_2)|\\
      = |b - s_1(c) + \lambda \cdot F(\SUCC(s_1, \alpha)) 
      - (b - s_2(c)) - \lambda \cdot F(\SUCC(s_2, \alpha))|\\
      = |(s_2(c) - s_1(c)) + \lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha)))|\\
      = |\lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha)))|\\
      \leq \lambda \cdot k \cdot \InfNorm{\SUCC(s_1, \alpha) -
        \SUCC(s_2, \alpha)}\\
      = \lambda \cdot k \cdot d
      = \lambda \cdot k \cdot \InfNorm{s_1 - s_2}
    \end{multline*}
    It follows that $F^\oplus_{\alpha, \lambda}$ is a contraction. 
    To prove that it is also monotonically decreasing, we need to show
    that $F^\oplus_{\alpha,\lambda}(s_1) -
    F^\oplus_{\alpha,\lambda}(s_2)$ is positive.
    \begin{multline*}
      F^\oplus_{\alpha,\lambda}(s_1) -
      F^\oplus_{\alpha,\lambda}(s_2)\\
      = b - s_1(c) + \lambda \cdot F(\SUCC(s_1, \alpha)) 
      - (b - s_2(c)) - \lambda \cdot F(\SUCC(s_2, \alpha))\\
      = \lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha))) \geq 0\\
    \end{multline*}
    The last inequality follows as $F$ is monotonically decreasing and
    $\SUCC(s_1, \alpha) \leq \SUCC(s_2, \alpha)$. 
    
  \item
    
    If $s_2(c) = s_1(c) + d$ then $\SUCC(s_2, \alpha) \leq \SUCC(s_1,
    \alpha)$ and moreover $\SUCC(s_1, \alpha) = \SUCC(s_2, \alpha) + d$.
    
    \begin{multline*}
      |F^\oplus_{\alpha,\lambda}(s_1) -
      F^\oplus_{\alpha,\lambda}(s_2)|\\
      = |b - s_1(c) + \lambda \cdot F(\SUCC(s_1, \alpha)) 
      - (b - s_2(c)) - \lambda \cdot F(\SUCC(s_2, \alpha))|\\
      = |(s_2(c) - s_1(c)) + \lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha)))|\\
      = |d + \lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha)))|\\
      \leq d = \InfNorm{s_1 - s_2}.
    \end{multline*}
    
    The inequality follows from the fact that $F$ is monotonically
    decreasing and $\SUCC(s_1,\alpha) \geq \SUCC(s_2, \alpha)$.
    We have thus shown that in this case $F^\oplus_{\alpha, \lambda}$
    is a contraction.  
    Again, to prove that it is also monotonically decreasing, we need
    to show that $F^\oplus_{\alpha,\lambda}(s_1) -
    F^\oplus_{\alpha,\lambda}(s_2)$ is positive. 
    
    \begin{multline*}
      F^\oplus_{\alpha,\lambda}(s_1) -
      F^\oplus_{\alpha,\lambda}(s_2)\\
      = b - s_1(c) + \lambda \cdot F(\SUCC(s_1, \alpha)) 
      - (b - s_2(c)) - \lambda \cdot F(\SUCC(s_2, \alpha))\\
      = d + \lambda \cdot (F(\SUCC(s_1, \alpha)) 
      -  F(\SUCC(s_2, \alpha))) \geq 0\\
    \end{multline*}
    The last inequality follows as $F$ is monotonically decreasing and
    $\SUCC(s_2, \alpha) \leq \SUCC(s_1, \alpha)$ and $F$ is a
    contraction. 

